Skill dependencies uncover nested human capital

Modern economies require increasingly diverse and specialized skills, many of which depend on the acquisition of other skills first. Here we analyse US survey data to reveal a nested structure within skill portfolios, where the direction of dependency is inferred from asymmetrical conditional probabilities-occupations require one skill conditional on another. This directional nature suggests that advanced, specific skills and knowledge are often built upon broader, fundamental ones. We examine 70 million job transitions to show that human capital development and career progression follow this structured pathway in which skills more aligned with the nested structure command higher wage premiums, require longer education and are less likely to be automated. These disparities are evident across genders and racial-ethnic groups, explaining long-term wage penalties. Finally, we find that this nested structure has become even more pronounced over the past two decades, indicating increased barriers to upward job mobility.

==> Nature_HB_2023/tabsNHB/Apr_1_2024_Wage_Regression_on_Skill_Endowments.tex <==
\begin{tabular}{@{\extracolsep{5pt}}lD{.}{.}{-3} D{.}{.}{-3} D{.}{.}{-3} D{.}{.}{-3} D{.}{.}{-3} D{.}{.}{-3} D{.}{.}{-3} } 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{7}{c}{\textit{Dependent variable:}} \\ 
\cline{2-8} 
\\[-1.8ex] & \multicolumn{7}{c}{Log(Mean Annual Wage)} \\ 
\\[-1.8ex] & \multicolumn{1}{c}{(1)} & \multicolumn{1}{c}{(2)} & \multicolumn{1}{c}{(3)} & \multicolumn{1}{c}{(4)} & \multicolumn{1}{c}{(5)} & \multicolumn{1}{c}{(6)} & \multicolumn{1}{c}{(7)}\\ 
\hline \\[-1.8ex] 
 General & 0.251^{***} &  &  & 0.135^{***} &  &  &  \\ 
  & \multicolumn{1}{c}{(0.237$, $0.264)} &  &  & \multicolumn{1}{c}{(0.109$, $0.161)} &  &  &  \\ 
  & & & & & & & \\ 
 Nested\_Intermediate &  & 0.261^{***} &  &  & 0.128^{***} &  &  \\ 
  &  & \multicolumn{1}{c}{(0.247$, $0.276)} &  &  & \multicolumn{1}{c}{(0.106$, $0.150)} &  &  \\ 
  & & & & & & & \\ 
 Unnested\_Intermediate &  & -0.003 &  &  & 0.025^{***} &  &  \\ 
  &  & \multicolumn{1}{c}{(-0.016$, $0.010)} &  &  & \multicolumn{1}{c}{(0.010$, $0.039)} &  &  \\ 
  & & & & & & & \\ 
 Nested\_Specific &  &  & 0.199^{***} &  &  & 0.042^{***} &  \\ 
  &  &  & \multicolumn{1}{c}{(0.182$, $0.215)} &  &  & \multicolumn{1}{c}{(0.020$, $0.064)} &  \\ 
  & & & & & & & \\ 
 Unnested\_Specific &  &  & -0.051^{***} &  &  & 0.003 &  \\ 
  &  &  & \multicolumn{1}{c}{(-0.063$, $-0.039)} &  &  & \multicolumn{1}{c}{(-0.011$, $0.017)} &  \\ 
  & & & & & & & \\ 
 Education &  &  &  & 0.024^{***} & 0.033^{***} & 0.042^{***} & 0.049^{***} \\ 
  &  &  &  & \multicolumn{1}{c}{(0.018$, $0.030)} & \multicolumn{1}{c}{(0.027$, $0.038)} & \multicolumn{1}{c}{(0.036$, $0.048)} & \multicolumn{1}{c}{(0.045$, $0.052)} \\ 
  & & & & & & & \\ 
 Experience &  &  &  & 0.014^{***} & 0.013^{***} & 0.023^{***} & 0.023^{***} \\ 
  &  &  &  & \multicolumn{1}{c}{(0.008$, $0.021)} & \multicolumn{1}{c}{(0.007$, $0.020)} & \multicolumn{1}{c}{(0.016$, $0.030)} & \multicolumn{1}{c}{(0.017$, $0.030)} \\ 
  & & & & & & & \\ 
 InJobTraining &  &  &  & 0.038^{***} & 0.027^{***} & 0.042^{***} & 0.048^{***} \\ 
  &  &  &  & \multicolumn{1}{c}{(0.029$, $0.048)} & \multicolumn{1}{c}{(0.017$, $0.037)} & \multicolumn{1}{c}{(0.031$, $0.052)} & \multicolumn{1}{c}{(0.039$, $0.058)} \\ 
  & & & & & & & \\ 
 Constant & 3.909^{***} & 4.109^{***} & 4.550^{***} & 3.969^{***} & 4.058^{***} & 4.223^{***} & 4.227^{***} \\ 
  & \multicolumn{1}{c}{(3.861$, $3.956)} & \multicolumn{1}{c}{(4.058$, $4.160)} & \multicolumn{1}{c}{(4.520$, $4.581)} & \multicolumn{1}{c}{(3.908$, $4.031)} & \multicolumn{1}{c}{(4.011$, $4.104)} & \multicolumn{1}{c}{(4.182$, $4.264)} & \multicolumn{1}{c}{(4.190$, $4.265)} \\ 
  & & & & & & & \\ 
\hline \\[-1.8ex] 
Observations & \multicolumn{1}{c}{789} & \multicolumn{1}{c}{789} & \multicolumn{1}{c}{789} & \multicolumn{1}{c}{789} & \multicolumn{1}{c}{789} & \multicolumn{1}{c}{789} & \multicolumn{1}{c}{789} \\ 
R$^{2}$ & \multicolumn{1}{c}{0.622} & \multicolumn{1}{c}{0.623} & \multicolumn{1}{c}{0.470} & \multicolumn{1}{c}{0.686} & \multicolumn{1}{c}{0.705} & \multicolumn{1}{c}{0.653} & \multicolumn{1}{c}{0.645} \\ 
Adjusted R$^{2}$ & \multicolumn{1}{c}{0.622} & \multicolumn{1}{c}{0.622} & \multicolumn{1}{c}{0.469} & \multicolumn{1}{c}{0.684} & \multicolumn{1}{c}{0.703} & \multicolumn{1}{c}{0.651} & \multicolumn{1}{c}{0.643} \\ 
Residual Std. Error & \multicolumn{1}{c}{0.119 (df = 787)} & \multicolumn{1}{c}{0.119 (df = 786)} & \multicolumn{1}{c}{0.142 (df = 786)} & \multicolumn{1}{c}{0.109 (df = 784)} & \multicolumn{1}{c}{0.106 (df = 783)} & \multicolumn{1}{c}{0.115 (df = 783)} & \multicolumn{1}{c}{0.116 (df = 785)} \\ 
F Statistic & \multicolumn{1}{c}{1,297.040$^{***}$ (df = 1; 787)} & \multicolumn{1}{c}{649.424$^{***}$ (df = 2; 786)} & \multicolumn{1}{c}{348.362$^{***}$ (df = 2; 786)} & \multicolumn{1}{c}{428.084$^{***}$ (df = 4; 784)} & \multicolumn{1}{c}{374.552$^{***}$ (df = 5; 783)} & \multicolumn{1}{c}{294.761$^{***}$ (df = 5; 783)} & \multicolumn{1}{c}{475.021$^{***}$ (df = 3; 785)} \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{7}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> Nature_HB_2023/tabsNHB/Aug_5_2023_-_Skill_Split_-_Nc_Nestedness_Simul_Aug_2023.tex <==
\begin{longtable}{@{\extracolsep{5pt}} 
    p{3cm}|p{12cm}}
    \caption{\textbf{The Skill Split Resulting from Nested Contribution of Skills based on $N_c$ \cite{write1992}.}} 
    \label{tab:skill_split_Nc_nestedness}
\\[-1.8ex]\hline 

\hline \\[-1.8ex] 
 Skill Category & Skill Titles \\ 
\hline \\[-1.8ex]
 \vspace{0.1 cm} \\
\endhead
Nested Specific (18 skills) & Biology, Chemistry, Design, Fine Arts, Foreign Language, Geography, History and Archeology, Management of Financial Resources, Management of Material Resources, Medicine and Dentistry, Philosophy and Theology, Physics, Programming, Science, Sociology and Anthropology, Technology Design, Telecommunications, Therapy and Counseling \\ 

\vspace{0.5 cm} \\
\hline \\[-1.8ex]

Un-nested Specific (28 skills) & Building and Construction, Dynamic Flexibility, Dynamic Strength, Equipment Maintenance, Equipment Selection, Explosive Strength, Extent Flexibility, Food Production, Glare Sensitivity, Gross Body Coordination, Gross Body Equilibrium, Installation, Mechanical, Multilimb Coordination, Night Vision, Operation and Control, Peripheral Vision, Rate Control, Reaction Time, Repairing, Response Orientation, Sound Localization, Spatial Orientation, Speed of Limb Movement, Stamina, Static Strength, Troubleshooting, Wrist-Finger Speed \\ 

\vspace{0.5 cm} \\
\hline \\[-1.8ex]

Nested Intermediate (26 skills) & Communications and Media, Economics and Accounting, Engineering and Technology, Far Vision, Flexibility of Closure, Fluency of Ideas, Instructing, Law and Government, Learning Strategies, Management of Personnel Resources, Mathematical Reasoning, Mathematics Skills, Memorization, Negotiation, Number Facility, Operations Analysis, Originality, Personnel and Human Resources, Persuasion, Psychology, Sales and Marketing, Selective Attention, Service Orientation, Speed of Closure, Systems Analysis, Systems Evaluation \\  

\vspace{0.5 cm} \\
\hline \\[-1.8ex]

Un-nested Intermediate (17 skills) & Arm-Hand Steadiness, Auditory Attention, Control Precision, Depth Perception, Finger Dexterity, Hearing Sensitivity, Manual Dexterity, Operation Monitoring, Perceptual Speed, Production and Processing, Public Safety and Security, Quality Control Analysis, Time Sharing, Transportation, Trunk Strength, Visual Color Discrimination, Visualization \\

\vspace{0.5 cm} \\
\hline \\[-1.8ex]

General (31 skills) & Active Learning, Active Listening, Administration and Management, Category Flexibility, Clerical, Complex Problem Solving, Computers and Electronics, Coordination, Critical Thinking, Customer and Personal Service, Deductive Reasoning, Education and Training, English Language, Inductive Reasoning, Information Ordering, Judgment and Decision Making, Mathematics Knowledge, Monitoring, Near Vision, Oral Comprehension, Oral Expression, Problem Sensitivity, Reading Comprehension, Social Perceptiveness, Speaking, Speech Clarity, Speech Recognition, Time Management, Writing, Written Comprehension, Written Expression \\ 
\vspace{0.5 cm} \\
\hline \\[-1.8ex] 
\end{longtable}

==> Nature_HB_2023/tabsNHB/May_28_-_SOC_OCC_2000-2010_Mismatch.tex <==
\begin{longtable}{@{\extracolsep{5pt}} 
    % {\centering}m{.1\textwidth}>
    % {\centering}m{.1\textwidth}>
    % {\raggedright\arraybackslash}m{.4\textwidth}>
    % {\centering}m{.1\textwidth}>
    % {\raggedright\arraybackslash}m{.4\textwidth}
    % cclcl}
    p{0.5cm}p{2cm}p{4.25cm}p{2cm}p{4.25cm}}
    \caption{List of SOC Code and Title Changes Between SOC 2000 (2003 data) and SOC 2010 (2019 data).} 
    \label{tab:list of onet soc changes}
\\[-1.8ex]\hline 

\hline \\[-1.8ex] 
 & $\text{SOC}_{2000}$ & $\text{SOC Title}_{2000}$ & $\text{SOC}_{2010}$ & $\text{SOC Title}_{2010}$ \\ 
\hline \\[-1.8ex] 

\endhead
1 & 11-1011.01 & Government Service Executives & 11-1011.00 & Chief Executives \\ 
2 & 11-1011.02 & Private Sector Executives & 11-1011.00 & Chief Executives \\ 
3 & 11-3040.00 & Human Resources Managers & 11-3121.00 & Human Resources Managers \\ 
4 & 11-3041.00 & Compensation and Benefits Managers & 11-3111.00 & Compensation and Benefits Managers \\ 
5 & 11-3042.00 & Training and Development Managers & 11-3131.00 & Training and Development Managers \\ 
6 & 11-3049.99 & Human Resources Managers, All Other & 11-3121.00 & Human Resources Managers \\ 
7 & 11-9011.00 & Farm, Ranch, and Other Agricultural Managers & 11-9013.00 &  \\ 
8 & 11-9011.01 & Nursery and Greenhouse Managers & 11-9013.01 & Nursery and Greenhouse Managers \\ 
9 & 11-9011.02 & Agricultural Crop Farm Managers & 11-9013.02 & Farm and Ranch Managers \\ 
10 & 11-9011.03 & Fish Hatchery Managers & 11-9013.03 & Aquacultural Managers \\ 
11 & 11-9012.00 & Farmers and Ranchers & 11-9013.02 & Farm and Ranch Managers \\ 
12 & 11-9039.99 & Education Administrators, All Other & 11-9039.00 &  \\ 
13 & 11-9061.00 & Funeral Directors & 39-4031.00 & Morticians, Undertakers, and Funeral Directors \\ 
14 & 11-9199.99 & Managers, All Other & 11-9199.00 &  \\ 
15 & 13-1041.05 & Pressure Vessel Inspectors & 47-4011.00 & Construction and Building Inspectors \\ 
16 & 13-1061.00 & Emergency Management Specialists & 11-9161.00 & Emergency Management Directors \\ 
17 & 13-1071.01 & Employment Interviewers, Private or Public Employment Service & 13-1071.00 & Human Resources Specialists \\ 
18 & 13-1071.02 & Personnel Recruiters & 13-1071.00 & Human Resources Specialists \\ 
19 & 13-1072.00 & Compensation, Benefits, and Job Analysis Specialists & 13-1141.00 & Compensation, Benefits, and Job Analysis Specialists \\ 
20 & 13-1073.00 & Training and Development Specialists & 13-1151.00 & Training and Development Specialists \\ 
21 & 13-1079.99 & Human Resources, Training, and Labor Relations Specialists, All Other & 13-1071.00 & Human Resources Specialists \\ 
22 & 13-1079.99 & Human Resources, Training, and Labor Relations Specialists, All Other & 13-1075.00 & Labor Relations Specialists \\ 
23 & 13-1199.99 & Business Operations Specialists, All Other & 13-1199.00 &  \\ 
24 & 13-2071.00 & Loan Counselors & 13-2071.01 & Loan Counselors \\ 
25 & 13-2099.99 & Financial Specialists, All Other & 13-2099.00 &  \\ 
26 & 15-1011.00 & Computer and Information Scientists, Research & 15-1111.00 & Computer and Information Research Scientists \\ 
27 & 15-1021.00 & Computer Programmers & 15-1131.00 & Computer Programmers \\ 
28 & 15-1031.00 & Computer Software Engineers, Applications & 15-1132.00 & Software Developers, Applications \\ 
29 & 15-1032.00 & Computer Software Engineers, Systems Software & 15-1133.00 & Software Developers, Systems Software \\ 
30 & 15-1041.00 & Computer Support Specialists & 15-1151.00 & Computer User Support Specialists \\ 
31 & 15-1051.00 & Computer Systems Analysts & 15-1121.00 & Computer Systems Analysts \\ 
32 & 15-1061.00 & Database Administrators & 15-1141.00 & Database Administrators \\ 
33 & 15-1071.00 & Network and Computer Systems Administrators & 15-1142.00 & Network and Computer Systems Administrators \\ 
34 & 15-1071.01 & Computer Security Specialists & 15-1122.00 & Information Security Analysts \\ 
35 & 15-1081.00 & Network Systems and Data Communications Analysts & 15-1143.00 & Computer Network Architects \\ 
36 & 15-1081.00 & Network Systems and Data Communications Analysts & 15-1152.00 & Computer Network Support Specialists \\ 
37 & 15-1099.99 & Computer Specialists, All Other & 15-1199.00 &  \\ 
38 & 15-2099.99 & Mathematical Science Occupations, All Other & 15-2099.00 &  \\ 
39 & 17-2199.99 & Engineers, All Other & 17-2199.00 &  \\ 
40 & 17-3019.99 & Drafters, All Other & 17-3019.00 &  \\ 
41 & 17-3023.02 & Calibration and Instrumentation Technicians & 17-3023.01 & Electronics Engineering Technicians \\ 
42 & 17-3029.99 & Engineering Technicians, Except Drafters, All Other & 17-3029.00 &  \\ 
43 & 19-1013.01 & Plant Scientists & 19-1013.00 & Soil and Plant Scientists \\ 
44 & 19-1013.02 & Soil Scientists & 19-1013.00 & Soil and Plant Scientists \\ 
45 & 19-1021.01 & Biochemists & 19-1021.00 & Biochemists and Biophysicists \\ 
46 & 19-1021.02 & Biophysicists & 19-1021.00 & Biochemists and Biophysicists \\ 
47 & 19-1029.99 & Biological Scientists, All Other & 19-1029.00 &  \\ 
48 & 19-1099.99 & Life Scientists, All Other & 19-1099.00 &  \\ 
49 & 19-2042.01 & Geologists & 19-2042.00 & Geoscientists, Except Hydrologists and Geographers \\ 
50 & 19-2099.99 & Physical Scientists, All Other & 19-2099.00 &  \\ 
51 & 19-3021.00 & Market Research Analysts & 13-1161.00 & Market Research Analysts and Marketing Specialists \\ 
52 & 19-3039.99 & Psychologists, All Other & 19-3039.00 &  \\ 
53 & 19-3099.99 & Social Scientists and Related Workers, All Other & 19-3099.00 &  \\ 
54 & 19-4099.99 & Life, Physical, and Social Science Technicians, All Other & 19-4099.00 &  \\ 
55 & 21-1019.99 & Counselors, All Other & 21-1019.00 &  \\ 
56 & 21-1029.99 & Social Workers, All Other & 21-1029.00 &  \\ 
57 & 21-1099.99 & Community and Social Service Specialists, All Other & 21-1099.00 &  \\ 
58 & 21-2099.99 & Religious Workers, All Other & 21-2099.00 &  \\ 
59 & 23-2092.00 & Law Clerks & 23-1012.00 & Judicial Law Clerks \\ 
60 & 23-2092.00 & Law Clerks & 23-2011.00 & Paralegals and Legal Assistants \\ 
61 & 23-2093.01 & Title Searchers & 23-2093.00 & Title Examiners, Abstractors, and Searchers \\ 
62 & 23-2093.02 & Title Examiners and Abstractors & 23-2093.00 & Title Examiners, Abstractors, and Searchers \\ 
63 & 23-2099.99 & Legal Support Workers, All Other & 23-2099.00 &  \\ 
64 & 25-1069.99 & Social Sciences Teachers, Postsecondary, All Other & 25-1069.00 &  \\ 
65 & 25-1199.99 & Postsecondary Teachers, All Other & 25-1199.00 &  \\ 
66 & 25-2041.00 & Special Education Teachers, Preschool, Kindergarten, and Elementary School & 25-2051.00 & Special Education Teachers, Preschool \\ 
67 & 25-2041.00 & Special Education Teachers, Preschool, Kindergarten, and Elementary School & 25-2052.00 & Special Education Teachers, Kindergarten and Elementary School \\ 
68 & 25-2042.00 & Special Education Teachers, Middle School & 25-2053.00 & Special Education Teachers, Middle School \\ 
69 & 25-2043.00 & Special Education Teachers, Secondary School & 25-2054.00 & Special Education Teachers, Secondary School \\ 
70 & 25-3099.99 & Teachers and Instructors, All Other & 25-3099.00 &  \\ 
71 & 25-9099.99 & Education, Training, and Library Workers, All Other & 25-9099.00 &  \\ 
72 & 27-1013.01 & Painters and Illustrators & 27-1013.00 & Fine Artists, Including Painters, Sculptors, and Illustrators \\ 
73 & 27-1013.02 & Sketch Artists & 27-1013.00 & Fine Artists, Including Painters, Sculptors, and Illustrators \\ 
74 & 27-1013.03 & Cartoonists & 27-1013.00 & Fine Artists, Including Painters, Sculptors, and Illustrators \\ 
75 & 27-1013.04 & Sculptors & 27-1013.00 & Fine Artists, Including Painters, Sculptors, and Illustrators \\ 
76 & 27-1019.99 & Artists and Related Workers, All Other & 27-1019.00 &  \\ 
77 & 27-1027.01 & Set Designers & 27-1027.00 & Set and Exhibit Designers \\ 
78 & 27-1027.02 & Exhibit Designers & 27-1027.00 & Set and Exhibit Designers \\ 
79 & 27-1029.99 & Designers, All Other & 27-1029.00 &  \\ 
80 & 27-2041.02 & Music Arrangers and Orchestrators & 27-2041.04 & Music Composers and Arrangers \\ 
81 & 27-2041.03 & Composers & 27-2041.04 & Music Composers and Arrangers \\ 
82 & 27-2099.99 & Entertainers and Performers, Sports and Related Workers, All Other & 27-2099.00 &  \\ 
83 & 27-3043.01 & Poets and Lyricists & 27-3043.05 & Poets, Lyricists and Creative Writers \\ 
84 & 27-3043.02 & Creative Writers & 27-3043.05 & Poets, Lyricists and Creative Writers \\ 
85 & 27-3043.03 & Caption Writers & 23-2091.00 & Court Reporters \\ 
86 & 27-3099.99 & Media and Communication Workers, All Other & 27-3099.00 &  \\ 
87 & 27-4021.01 & Professional Photographers & 27-4021.00 & Photographers \\ 
88 & 27-4021.02 & Photographers, Scientific & 27-4021.00 & Photographers \\ 
89 & 27-4099.99 & Media and Communication Equipment Workers, All Other & 27-4099.00 &  \\ 
90 & 29-1029.99 & Dentists, All Other Specialists & 29-1029.00 &  \\ 
91 & 29-1069.99 & Physicians and Surgeons, All Other & 29-1069.00 &  \\ 
92 & 29-1111.00 & Registered Nurses & 29-1141.00 & Registered Nurses \\ 
93 & 29-1121.00 & Audiologists & 29-1181.00 & Audiologists \\ 
94 & 29-1129.99 & Therapists, All Other & 29-1129.00 &  \\ 
95 & 29-1199.99 & Health Diagnosing and Treating Practitioners, All Other & 29-1199.00 &  \\ 
96 & 29-2034.00 & Radiologic Technologists and Technicians & 29-2099.06 & Radiologic Technicians \\ 
97 & 29-2034.01 & Radiologic Technologists & 29-2034.00 & Radiologic Technologists \\ 
98 & 29-2034.02 & Radiologic Technicians & 29-2099.06 & Radiologic Technicians \\ 
99 & 29-2099.99 & Health Technologists and Technicians, All Other & 29-2099.00 &  \\ 
100 & 29-9099.99 & Healthcare Practitioners and Technical Workers, All Other & 29-9099.00 &  \\ 
101 & 31-1012.00 & Nursing Aides, Orderlies, and Attendants & 31-1014.00 & Nursing Assistants \\ 
102 & 31-1012.00 & Nursing Aides, Orderlies, and Attendants & 31-1015.00 & Orderlies \\ 
103 & 31-9099.99 & Healthcare Support Workers, All Other & 31-9099.00 &  \\ 
104 & 33-1099.99 & First-Line Supervisors/Managers, Protective Service Workers, All Other & 33-1099.00 &  \\ 
105 & 33-3021.04 & Child Support, Missing Persons, and Unemployment Insurance Fraud Investigators & 33-3021.03 & Criminal Investigators and Special Agents \\ 
106 & 33-3051.02 & Highway Patrol Pilots & 33-3051.01 & Police Patrol Officers \\ 
107 & 33-9099.99 & Protective Service Workers, All Other & 33-9099.00 &  \\ 
108 & 35-2019.99 & Cooks, All Other & 35-2019.00 &  \\ 
109 & 35-9099.99 & Food Preparation and Serving Related Workers, All Other & 35-9099.00 &  \\ 
110 & 37-1011.01 & Housekeeping Supervisors & 37-1011.00 & First-Line Supervisors of Housekeeping and Janitorial Workers \\ 
111 & 37-1011.02 & Janitorial Supervisors & 37-1011.00 & First-Line Supervisors of Housekeeping and Janitorial Workers \\ 
112 & 37-1012.01 & Lawn Service Managers & 37-1012.00 & First-Line Supervisors of Landscaping, Lawn Service, and Groundskeeping Workers \\ 
113 & 37-1012.02 & First-Line Supervisors and Manager/Supervisors - Landscaping Workers & 37-1012.00 & First-Line Supervisors of Landscaping, Lawn Service, and Groundskeeping Workers \\ 
114 & 37-2019.99 & Building Cleaning Workers, All Other & 37-2019.00 &  \\ 
115 & 37-3019.99 & Grounds Maintenance Workers, All Other & 37-3019.00 &  \\ 
116 & 39-3019.99 & Gaming Service Workers, All Other & 39-3019.00 &  \\ 
117 & 39-3099.99 & Entertainment Attendants and Related Workers, All Other & 39-3099.00 &  \\ 
118 & 39-6021.00 & Tour Guides and Escorts & 39-7011.00 & Tour Guides and Escorts \\ 
119 & 39-6022.00 & Travel Guides & 39-7012.00 & Travel Guides \\ 
120 & 39-6031.00 & Flight Attendants & 53-2031.00 & Flight Attendants \\ 
121 & 39-6032.00 & Transportation Attendants, Except Flight Attendants and Baggage Porters & 53-6061.00 & Transportation Attendants, Except Flight Attendants \\ 
122 & 39-9099.99 & Personal Care and Service Workers, All Other & 39-9099.00 &  \\ 
123 & 41-3099.99 & Sales Representatives, Services, All Other & 41-3099.00 &  \\ 
124 & 41-4011.01 & Sales Representatives, Agricultural & 41-4011.00 & Sales Representatives, Wholesale and Manufacturing, Technical and Scientific Products \\ 
125 & 41-4011.02 & Sales Representatives, Chemical and Pharmaceutical & 41-4011.00 & Sales Representatives, Wholesale and Manufacturing, Technical and Scientific Products \\ 
126 & 41-4011.03 & Sales Representatives, Electrical/Electronic & 41-4011.00 & Sales Representatives, Wholesale and Manufacturing, Technical and Scientific Products \\ 
127 & 41-4011.04 & Sales Representatives, Mechanical Equipment and Supplies & 41-4011.00 & Sales Representatives, Wholesale and Manufacturing, Technical and Scientific Products \\ 
128 & 41-4011.05 & Sales Representatives, Medical & 41-4011.00 & Sales Representatives, Wholesale and Manufacturing, Technical and Scientific Products \\ 
129 & 41-4011.06 & Sales Representatives, Instruments & 41-4011.00 & Sales Representatives, Wholesale and Manufacturing, Technical and Scientific Products \\ 
130 & 41-9099.99 & Sales and Related Workers, All Other & 41-9099.00 &  \\ 
131 & 43-1011.01 & First-Line Supervisors, Customer Service & 43-1011.00 & First-Line Supervisors of Office and Administrative Support Workers \\ 
132 & 43-1011.02 & First-Line Supervisors, Administrative Support & 43-1011.00 & First-Line Supervisors of Office and Administrative Support Workers \\ 
133 & 43-2021.01 & Directory Assistance Operators & 43-2021.00 & Telephone Operators \\ 
134 & 43-2021.02 & Central Office Operators & 43-2021.00 & Telephone Operators \\ 
135 & 43-2099.99 & Communications Equipment Operators, All Other & 43-2099.00 &  \\ 
136 & 43-3021.03 & Billing, Posting, and Calculating Machine Operators & 43-3021.00 &  \\ 
137 & 43-4051.01 & Adjustment Clerks & 43-4051.00 & Customer Service Representatives \\ 
138 & 43-4051.02 & Customer Service Representatives, Utilities & 43-4051.00 & Customer Service Representatives \\ 
139 & 43-4061.01 & Claims Takers, Unemployment Benefits & 43-4061.00 & Eligibility Interviewers, Government Programs \\ 
140 & 43-4061.02 & Welfare Eligibility Workers and Interviewers & 43-4061.00 & Eligibility Interviewers, Government Programs \\ 
141 & 43-4181.01 & Travel Clerks & 43-4181.00 & Reservation and Transportation Ticket Agents and Travel Clerks \\ 
142 & 43-4181.02 & Reservation and Transportation Ticket Agents & 43-4181.00 & Reservation and Transportation Ticket Agents and Travel Clerks \\ 
143 & 43-4199.99 & Information and Record Clerks, All Other & 43-4199.00 &  \\ 
144 & 43-9051.01 & Mail Machine Operators, Preparation and Handling & 43-9051.00 & Mail Clerks and Mail Machine Operators, Except Postal Service \\ 
145 & 43-9051.02 & Mail Clerks, Except Mail Machine Operators and Postal Service & 43-9051.00 & Mail Clerks and Mail Machine Operators, Except Postal Service \\ 
146 & 43-9071.01 & Duplicating Machine Operators & 43-9071.00 & Office Machine Operators, Except Computer \\ 
147 & 43-9199.99 & Office and Administrative Support Workers, All Other & 43-9199.00 &  \\ 
148 & 45-1011.01 & First-Line Supervisors and Manager/Supervisors - Agricultural Crop Workers & 45-1011.07 & First-Line Supervisors of Agricultural Crop and Horticultural Workers \\ 
149 & 45-1011.02 & First-Line Supervisors and Manager/Supervisors - Animal Husbandry Workers & 45-1011.08 & First-Line Supervisors of Animal Husbandry and Animal Care Workers \\ 
150 & 45-1011.03 & First-Line Supervisors and Manager/Supervisors - Animal Care Workers, Except Livestock & 45-1011.08 & First-Line Supervisors of Animal Husbandry and Animal Care Workers \\ 
151 & 45-1011.04 & First-Line Supervisors and Manager/Supervisors - Horticultural Workers & 45-1011.07 & First-Line Supervisors of Agricultural Crop and Horticultural Workers \\ 
152 & 45-1012.00 & Farm Labor Contractors & 13-1074.00 & Farm Labor Contractors \\ 
153 & 45-2099.99 & Agricultural Workers, All Other & 45-2099.00 &  \\ 
154 & 45-4022.01 & Logging Tractor Operators & 45-4022.00 & Logging Equipment Operators \\ 
155 & 45-4029.99 & Logging Workers, All Other & 45-4029.00 &  \\ 
156 & 47-1011.01 & First-Line Supervisors and Manager/Supervisors- Construction Trades Workers & 47-1011.00 & First-Line Supervisors of Construction Trades and Extraction Workers \\ 
157 & 47-1011.02 & First-Line Supervisors and Manager/Supervisors- Extractive Workers & 47-1011.00 & First-Line Supervisors of Construction Trades and Extraction Workers \\ 
158 & 47-2031.03 & Carpenter Assemblers and Repairers & 47-2031.01 & Construction Carpenters \\ 
159 & 47-2031.04 & Ship Carpenters and Joiners & 47-2031.01 & Construction Carpenters \\ 
160 & 47-2031.05 & Boat Builders and Shipwrights & 47-2031.01 & Construction Carpenters \\ 
161 & 47-2031.06 & Brattice Builders & 47-2031.02 & Rough Carpenters \\ 
162 & 47-2073.01 & Grader, Bulldozer, and Scraper Operators & 47-2073.00 & Operating Engineers and Other Construction Equipment Operators \\ 
163 & 47-2073.02 & Operating Engineers & 47-2073.00 & Operating Engineers and Other Construction Equipment Operators \\ 
164 & 47-2081.01 & Ceiling Tile Installers & 47-2081.00 & Drywall and Ceiling Tile Installers \\ 
165 & 47-2081.02 & Drywall Installers & 47-2081.00 & Drywall and Ceiling Tile Installers \\ 
166 & 47-2152.03 & Pipelaying Fitters & 47-2151.00 & Pipelayers \\ 
167 & 47-3019.99 & Helpers, Construction Trades, All Other & 47-3019.00 &  \\ 
168 & 47-4041.01 & Irradiated-Fuel Handlers & 47-4041.00 & Hazardous Materials Removal Workers \\ 
169 & 47-4099.99 & Construction and Related Workers, All Other & 47-4099.00 &  \\ 
170 & 47-5021.01 & Construction Drillers & 47-5021.00 & Earth Drillers, Except Oil and Gas \\ 
171 & 47-5021.02 & Well and Core Drill Operators & 47-5021.00 & Earth Drillers, Except Oil and Gas \\ 
172 & 47-5049.99 & Mining Machine Operators, All Other & 47-5049.00 &  \\ 
173 & 47-5099.99 & Extraction Workers, All Other & 47-5099.00 &  \\ 
174 & 49-2011.01 & Automatic Teller Machine Servicers & 49-9091.00 & Coin, Vending, and Amusement Machine Servicers and Repairers \\ 
175 & 49-2011.02 & Data Processing Equipment Repairers & 49-2011.00 & Computer, Automated Teller, and Office Machine Repairers \\ 
176 & 49-2011.03 & Office Machine and Cash Register Servicers & 49-2011.00 & Computer, Automated Teller, and Office Machine Repairers \\ 
177 & 49-2021.00 & Radio Mechanics & 49-2021.01 & Radio Mechanics \\ 
178 & 49-2022.01 & Central Office and PBX Installers and Repairers & 49-2022.00 & Telecommunications Equipment Installers and Repairers, Except Line Installers \\ 
179 & 49-2022.02 & Frame Wirers, Central Office & 49-2022.00 & Telecommunications Equipment Installers and Repairers, Except Line Installers \\ 
180 & 49-2022.03 & Communication Equipment Mechanics, Installers, and Repairers & 49-2022.00 & Telecommunications Equipment Installers and Repairers, Except Line Installers \\ 
181 & 49-2022.04 & Telecommunications Facility Examiners & 49-2022.00 & Telecommunications Equipment Installers and Repairers, Except Line Installers \\ 
182 & 49-2022.05 & Station Installers and Repairers, Telephone & 49-2022.00 & Telecommunications Equipment Installers and Repairers, Except Line Installers \\ 
183 & 49-2092.01 & Electric Home Appliance and Power Tool Repairers & 49-9031.00 & Home Appliance Repairers \\ 
184 & 49-2092.02 & Electric Motor and Switch Assemblers and Repairers & 49-2092.00 & Electric Motor, Power Tool, and Related Repairers \\ 
185 & 49-2092.03 & Battery Repairers & 49-2092.00 & Electric Motor, Power Tool, and Related Repairers \\ 
186 & 49-2092.04 & Transformer Repairers & 49-2092.00 & Electric Motor, Power Tool, and Related Repairers \\ 
187 & 49-2092.05 & Electrical Parts Reconditioners & 49-2092.00 & Electric Motor, Power Tool, and Related Repairers \\ 
188 & 49-2092.06 & Hand and Portable Power Tool Repairers & 49-2092.00 & Electric Motor, Power Tool, and Related Repairers \\ 
189 & 49-3011.01 & Airframe-and-Power-Plant Mechanics & 49-3011.00 & Aircraft Mechanics and Service Technicians \\ 
190 & 49-3011.02 & Aircraft Engine Specialists & 49-3011.00 & Aircraft Mechanics and Service Technicians \\ 
191 & 49-3011.03 & Aircraft Body and Bonded Structure Repairers & 49-3011.00 & Aircraft Mechanics and Service Technicians \\ 
192 & 49-9012.01 & Electric Meter Installers and Repairers & 49-9012.00 & Control and Valve Installers and Repairers, Except Mechanical Door \\ 
193 & 49-9012.02 & Valve and Regulator Repairers & 49-9012.00 & Control and Valve Installers and Repairers, Except Mechanical Door \\ 
194 & 49-9012.03 & Meter Mechanics & 49-9012.00 & Control and Valve Installers and Repairers, Except Mechanical Door \\ 
195 & 49-9031.01 & Home Appliance Installers & 49-9031.00 & Home Appliance Repairers \\ 
196 & 49-9031.02 & Gas Appliance Repairers & 49-9031.00 & Home Appliance Repairers \\ 
197 & 49-9042.00 & Maintenance and Repair Workers, General & 49-9071.00 & Maintenance and Repair Workers, General \\ 
198 & 49-9063.01 & Keyboard Instrument Repairers and Tuners & 49-9063.00 & Musical Instrument Repairers and Tuners \\ 
199 & 49-9063.02 & Stringed Instrument Repairers and Tuners & 49-9063.00 & Musical Instrument Repairers and Tuners \\ 
200 & 49-9063.03 & Reed or Wind Instrument Repairers and Tuners & 49-9063.00 & Musical Instrument Repairers and Tuners \\ 
201 & 49-9063.04 & Percussion Instrument Repairers and Tuners & 49-9063.00 & Musical Instrument Repairers and Tuners \\ 
202 & 49-9069.99 & Precision Instrument and Equipment Repairers, All Other & 49-9069.00 &  \\ 
203 & 49-9099.99 & Installation, Maintenance, and Repair Workers, All Other & 49-9099.00 &  \\ 
204 & 51-2011.01 & Aircraft Structure Assemblers, Precision & 51-2011.00 & Aircraft Structure, Surfaces, Rigging, and Systems Assemblers \\ 
205 & 51-2011.02 & Aircraft Systems Assemblers, Precision & 51-2011.00 & Aircraft Structure, Surfaces, Rigging, and Systems Assemblers \\ 
206 & 51-2011.03 & Aircraft Rigging Assemblers & 51-2011.00 & Aircraft Structure, Surfaces, Rigging, and Systems Assemblers \\ 
207 & 51-2041.01 & Metal Fabricators, Structural Metal Products & 51-2041.00 & Structural Metal Fabricators and Fitters \\ 
208 & 51-2041.02 & Fitters, Structural Metal- Precision & 51-2041.00 & Structural Metal Fabricators and Fitters \\ 
209 & 51-2099.99 & Assemblers and Fabricators, All Other & 51-2099.00 &  \\ 
210 & 51-3011.01 & Bakers, Bread and Pastry & 35-1011.00 & Chefs and Head Cooks \\ 
211 & 51-3011.02 & Bakers, Manufacturing & 51-3011.00 & Bakers \\ 
212 & 51-4011.01 & Numerical Control Machine Tool Operators and Tenders, Metal and Plastic & 51-4011.00 & Computer-Controlled Machine Tool Operators, Metal and Plastic \\ 
213 & 51-4031.01 & Sawing Machine Tool Setters and Set-Up Operators, Metal and Plastic & 51-4031.00 & Cutting, Punching, and Press Machine Setters, Operators, and Tenders, Metal and Plastic \\ 
214 & 51-4031.02 & Punching Machine Setters and Set-Up Operators, Metal and Plastic & 51-4031.00 & Cutting, Punching, and Press Machine Setters, Operators, and Tenders, Metal and Plastic \\ 
215 & 51-4031.03 & Press and Press Brake Machine Setters and Set-Up Operators, Metal and Plastic & 51-4031.00 & Cutting, Punching, and Press Machine Setters, Operators, and Tenders, Metal and Plastic \\ 
216 & 51-4031.04 & Shear and Slitter Machine Setters and Set-Up Operators, Metal and Plastic & 51-4031.00 & Cutting, Punching, and Press Machine Setters, Operators, and Tenders, Metal and Plastic \\ 
217 & 51-4033.01 & Grinding, Honing, Lapping, and Deburring Machine Set-Up Operators & 51-4033.00 & Grinding, Lapping, Polishing, and Buffing Machine Tool Setters, Operators, and Tenders, Metal and Plastic \\ 
218 & 51-4033.02 & Buffing and Polishing Set-Up Operators & 51-4033.00 & Grinding, Lapping, Polishing, and Buffing Machine Tool Setters, Operators, and Tenders, Metal and Plastic \\ 
219 & 51-4072.01 & Plastic Molding and Casting Machine Setters and Set-Up Operators & 51-4072.00 & Molding, Coremaking, and Casting Machine Setters, Operators, and Tenders, Metal and Plastic \\ 
220 & 51-4072.02 & Plastic Molding and Casting Machine Operators and Tenders & 51-4072.00 & Molding, Coremaking, and Casting Machine Setters, Operators, and Tenders, Metal and Plastic \\ 
221 & 51-4072.03 & Metal Molding, Coremaking, and Casting Machine Setters and Set-Up Operators & 51-4072.00 & Molding, Coremaking, and Casting Machine Setters, Operators, and Tenders, Metal and Plastic \\ 
222 & 51-4072.04 & Metal Molding, Coremaking, and Casting Machine Operators and Tenders & 51-4072.00 & Molding, Coremaking, and Casting Machine Setters, Operators, and Tenders, Metal and Plastic \\ 
223 & 51-4072.05 & Casting Machine Set-Up Operators & 51-4072.00 & Molding, Coremaking, and Casting Machine Setters, Operators, and Tenders, Metal and Plastic \\ 
224 & 51-4081.01 & Combination Machine Tool Setters and Set-Up Operators, Metal and Plastic & 51-4081.00 & Multiple Machine Tool Setters, Operators, and Tenders, Metal and Plastic \\ 
225 & 51-4081.02 & Combination Machine Tool Operators and Tenders, Metal and Plastic & 51-4081.00 & Multiple Machine Tool Setters, Operators, and Tenders, Metal and Plastic \\ 
226 & 51-4121.01 & Welders, Production & 51-4121.06 & Welders, Cutters, and Welder Fitters \\ 
227 & 51-4121.02 & Welders and Cutters & 51-4121.06 & Welders, Cutters, and Welder Fitters \\ 
228 & 51-4121.03 & Welder-Fitters & 51-4121.06 & Welders, Cutters, and Welder Fitters \\ 
229 & 51-4121.04 & Solderers & 51-4121.07 & Solderers and Brazers \\ 
230 & 51-4121.05 & Brazers & 51-4121.07 & Solderers and Brazers \\ 
231 & 51-4122.01 & Welding Machine Setters and Set-Up Operators & 51-4122.00 & Welding, Soldering, and Brazing Machine Setters, Operators, and Tenders \\ 
232 & 51-4122.02 & Welding Machine Operators and Tenders & 51-4122.00 & Welding, Soldering, and Brazing Machine Setters, Operators, and Tenders \\ 
233 & 51-4122.03 & Soldering and Brazing Machine Setters and Set-Up Operators & 51-4122.00 & Welding, Soldering, and Brazing Machine Setters, Operators, and Tenders \\ 
234 & 51-4122.04 & Soldering and Brazing Machine Operators and Tenders & 51-4122.00 & Welding, Soldering, and Brazing Machine Setters, Operators, and Tenders \\ 
235 & 51-4191.01 & Heating Equipment Setters and Set-Up Operators, Metal and Plastic & 51-4191.00 & Heat Treating Equipment Setters, Operators, and Tenders, Metal and Plastic \\ 
236 & 51-4191.02 & Heat Treating, Annealing, and Tempering Machine Operators and Tenders, Metal and Plastic & 51-4191.00 & Heat Treating Equipment Setters, Operators, and Tenders, Metal and Plastic \\ 
237 & 51-4191.03 & Heaters, Metal and Plastic & 51-4191.00 & Heat Treating Equipment Setters, Operators, and Tenders, Metal and Plastic \\ 
238 & 51-4193.01 & Electrolytic Plating and Coating Machine Setters and Set-Up Operators, Metal and Plastic & 51-4193.00 & Plating and Coating Machine Setters, Operators, and Tenders, Metal and Plastic \\ 
239 & 51-4193.02 & Electrolytic Plating and Coating Machine Operators and Tenders, Metal and Plastic & 51-4193.00 & Plating and Coating Machine Setters, Operators, and Tenders, Metal and Plastic \\ 
240 & 51-4193.03 & Nonelectrolytic Plating and Coating Machine Setters and Set-Up Operators, Metal and Plastic & 51-4193.00 & Plating and Coating Machine Setters, Operators, and Tenders, Metal and Plastic \\ 
241 & 51-4193.04 & Nonelectrolytic Plating and Coating Machine Operators and Tenders, Metal and Plastic & 51-4193.00 & Plating and Coating Machine Setters, Operators, and Tenders, Metal and Plastic \\ 
242 & 51-4199.99 & Metal Workers and Plastic Workers, All Other & 51-4199.00 &  \\ 
243 & 51-5011.00 & Bindery Workers & 51-5113.00 & Print Binding and Finishing Workers \\ 
244 & 51-5011.01 & Bindery Machine Setters and Set-Up Operators & 51-5113.00 & Print Binding and Finishing Workers \\ 
245 & 51-5011.02 & Bindery Machine Operators and Tenders & 51-5113.00 & Print Binding and Finishing Workers \\ 
246 & 51-5012.00 & Bookbinders & 51-5113.00 & Print Binding and Finishing Workers \\ 
247 & 51-5021.00 & Job Printers & 51-5112.00 & Printing Press Operators \\ 
248 & 51-5021.00 & Job Printers & 51-5113.00 & Print Binding and Finishing Workers \\ 
249 & 51-5022.00 & Prepress Technicians and Workers & 51-5111.00 & Prepress Technicians and Workers \\ 
250 & 51-5022.01 & Hand Compositors and Typesetters & 51-5111.00 & Prepress Technicians and Workers \\ 
251 & 51-5022.02 & Paste-Up Workers & 51-5111.00 & Prepress Technicians and Workers \\ 
252 & 51-5022.03 & Photoengravers & 51-5111.00 & Prepress Technicians and Workers \\ 
253 & 51-5022.04 & Camera Operators & 51-5111.00 & Prepress Technicians and Workers \\ 
254 & 51-5022.05 & Scanner Operators & 51-5111.00 & Prepress Technicians and Workers \\ 
255 & 51-5022.06 & Strippers & 51-5111.00 & Prepress Technicians and Workers \\ 
256 & 51-5022.07 & Platemakers & 51-5111.00 & Prepress Technicians and Workers \\ 
257 & 51-5022.08 & Dot Etchers & 51-5111.00 & Prepress Technicians and Workers \\ 
258 & 51-5022.09 & Electronic Masking System Operators & 51-5111.00 & Prepress Technicians and Workers \\ 
259 & 51-5022.10 & Electrotypers and Stereotypers & 51-5111.00 & Prepress Technicians and Workers \\ 
260 & 51-5022.11 & Plate Finishers & 51-5111.00 & Prepress Technicians and Workers \\ 
261 & 51-5022.12 & Typesetting and Composing Machine Operators and Tenders & 51-5111.00 & Prepress Technicians and Workers \\ 
262 & 51-5022.13 & Photoengraving and Lithographing Machine Operators and Tenders & 51-5111.00 & Prepress Technicians and Workers \\ 
263 & 51-5023.00 & Printing Machine Operators & 51-5112.00 & Printing Press Operators \\ 
264 & 51-5023.01 & Precision Printing Workers & 51-5112.00 & Printing Press Operators \\ 
265 & 51-5023.02 & Offset Lithographic Press Setters and Set-Up Operators & 51-5112.00 & Printing Press Operators \\ 
266 & 51-5023.03 & Letterpress Setters and Set-Up Operators & 51-5112.00 & Printing Press Operators \\ 
267 & 51-5023.04 & Design Printing Machine Setters and Set-Up Operators & 51-5112.00 & Printing Press Operators \\ 
268 & 51-5023.05 & Marking and Identification Printing Machine Setters and Set-Up Operators & 51-5112.00 & Printing Press Operators \\ 
269 & 51-5023.06 & Screen Printing Machine Setters and Set-Up Operators & 51-5112.00 & Printing Press Operators \\ 
270 & 51-5023.07 & Embossing Machine Set-Up Operators & 51-5112.00 & Printing Press Operators \\ 
271 & 51-5023.08 & Engraver Set-Up Operators & 51-5112.00 & Printing Press Operators \\ 
272 & 51-5023.09 & Printing Press Machine Operators and Tenders & 51-5112.00 & Printing Press Operators \\ 
273 & 51-6011.01 & Spotters, Dry Cleaning & 51-6011.00 & Laundry and Dry-Cleaning Workers \\ 
274 & 51-6011.02 & Precision Dyers & 51-6011.00 & Laundry and Dry-Cleaning Workers \\ 
275 & 51-6011.03 & Laundry and Drycleaning Machine Operators and Tenders, Except Pressing & 51-6011.00 & Laundry and Dry-Cleaning Workers \\ 
276 & 51-6021.01 & Pressers, Delicate Fabrics & 51-6021.00 & Pressers, Textile, Garment, and Related Materials \\ 
277 & 51-6021.02 & Pressing Machine Operators and Tenders- Textile, Garment, and Related Materials & 51-6021.00 & Pressers, Textile, Garment, and Related Materials \\ 
278 & 51-6021.03 & Pressers, Hand & 51-6021.00 & Pressers, Textile, Garment, and Related Materials \\ 
279 & 51-6031.01 & Sewing Machine Operators, Garment & 51-6031.00 & Sewing Machine Operators \\ 
280 & 51-6031.02 & Sewing Machine Operators, Non-Garment & 51-6031.00 & Sewing Machine Operators \\ 
281 & 51-6052.01 & Shop and Alteration Tailors & 51-6052.00 & Tailors, Dressmakers, and Custom Sewers \\ 
282 & 51-6052.02 & Custom Tailors & 51-6052.00 & Tailors, Dressmakers, and Custom Sewers \\ 
283 & 51-6091.01 & Extruding and Forming Machine Operators and Tenders, Synthetic or Glass Fibers & 51-6091.00 & Extruding and Forming Machine Setters, Operators, and Tenders, Synthetic and Glass Fibers \\ 
284 & 51-6099.99 & Textile, Apparel, and Furnishings Workers, All Other & 51-6099.00 &  \\ 
285 & 51-7041.01 & Sawing Machine Setters and Set-Up Operators & 51-7041.00 & Sawing Machine Setters, Operators, and Tenders, Wood \\ 
286 & 51-7041.02 & Sawing Machine Operators and Tenders & 51-7041.00 & Sawing Machine Setters, Operators, and Tenders, Wood \\ 
287 & 51-7042.01 & Woodworking Machine Setters and Set-Up Operators, Except Sawing & 51-7042.00 & Woodworking Machine Setters, Operators, and Tenders, Except Sawing \\ 
288 & 51-7042.02 & Woodworking Machine Operators and Tenders, Except Sawing & 51-7042.00 & Woodworking Machine Setters, Operators, and Tenders, Except Sawing \\ 
289 & 51-7099.99 & Woodworkers, All Other & 51-7099.00 &  \\ 
290 & 51-8013.01 & Power Generating Plant Operators, Except Auxiliary Equipment Operators & 51-8013.00 & Power Plant Operators \\ 
291 & 51-8013.02 & Auxiliary Equipment Operators, Power & 51-8013.00 & Power Plant Operators \\ 
292 & 51-8021.01 & Boiler Operators and Tenders, Low Pressure & 51-8021.00 & Stationary Engineers and Boiler Operators \\ 
293 & 51-8021.02 & Stationary Engineers & 51-8021.00 & Stationary Engineers and Boiler Operators \\ 
294 & 51-8092.01 & Gas Processing Plant Operators & 51-8092.00 & Gas Plant Operators \\ 
295 & 51-8092.02 & Gas Distribution Plant Operators & 51-8092.00 & Gas Plant Operators \\ 
296 & 51-8093.01 & Petroleum Pump System Operators & 51-8093.00 & Petroleum Pump System Operators, Refinery Operators, and Gaugers \\ 
297 & 51-8093.02 & Petroleum Refinery and Control Panel Operators & 51-8093.00 & Petroleum Pump System Operators, Refinery Operators, and Gaugers \\ 
298 & 51-8093.03 & Gaugers & 51-8093.00 & Petroleum Pump System Operators, Refinery Operators, and Gaugers \\ 
299 & 51-8099.99 & Plant and System Operators, All Other & 51-8099.00 &  \\ 
300 & 51-9011.01 & Chemical Equipment Controllers and Operators & 51-9011.00 & Chemical Equipment Operators and Tenders \\ 
301 & 51-9011.02 & Chemical Equipment Tenders & 51-9011.00 & Chemical Equipment Operators and Tenders \\ 
302 & 51-9032.01 & Fiber Product Cutting Machine Setters and Set-Up Operators & 51-9032.00 & Cutting and Slicing Machine Setters, Operators, and Tenders \\ 
303 & 51-9032.02 & Stone Sawyers & 51-9032.00 & Cutting and Slicing Machine Setters, Operators, and Tenders \\ 
304 & 51-9032.03 & Glass Cutting Machine Setters and Set-Up Operators & 51-9032.00 & Cutting and Slicing Machine Setters, Operators, and Tenders \\ 
305 & 51-9032.04 & Cutting and Slicing Machine Operators and Tenders & 51-9032.00 & Cutting and Slicing Machine Setters, Operators, and Tenders \\ 
306 & 51-9041.01 & Extruding, Forming, Pressing, and Compacting Machine Setters and Set-Up Operators & 51-9041.00 & Extruding, Forming, Pressing, and Compacting Machine Setters, Operators, and Tenders \\ 
307 & 51-9041.02 & Extruding, Forming, Pressing, and Compacting Machine Operators and Tenders & 51-9041.00 & Extruding, Forming, Pressing, and Compacting Machine Setters, Operators, and Tenders \\ 
308 & 51-9061.01 & Materials Inspectors & 51-9061.00 & Inspectors, Testers, Sorters, Samplers, and Weighers \\ 
309 & 51-9061.02 & Mechanical Inspectors & 51-9061.00 & Inspectors, Testers, Sorters, Samplers, and Weighers \\ 
310 & 51-9061.03 & Precision Devices Inspectors and Testers & 51-9061.00 & Inspectors, Testers, Sorters, Samplers, and Weighers \\ 
311 & 51-9061.04 & Electrical and Electronic Inspectors and Testers & 51-9061.00 & Inspectors, Testers, Sorters, Samplers, and Weighers \\ 
312 & 51-9061.05 & Production Inspectors, Testers, Graders, Sorters, Samplers, Weighers & 51-9061.00 & Inspectors, Testers, Sorters, Samplers, and Weighers \\ 
313 & 51-9071.02 & Silversmiths & 51-9071.07 & Precious Metal Workers \\ 
314 & 51-9071.03 & Model and Mold Makers, Jewelry & 51-9071.01 & Jewelers \\ 
315 & 51-9071.04 & Bench Workers, Jewelry & 51-9071.01 & Jewelers \\ 
316 & 51-9071.05 & Pewter Casters and Finishers & 51-9071.07 & Precious Metal Workers \\ 
317 & 51-9083.01 & Precision Lens Grinders and Polishers & 51-9083.00 & Ophthalmic Laboratory Technicians \\ 
318 & 51-9083.02 & Optical Instrument Assemblers & 51-9083.00 & Ophthalmic Laboratory Technicians \\ 
319 & 51-9121.01 & Coating, Painting, and Spraying Machine Setters and Set-Up Operators & 51-9121.00 & Coating, Painting, and Spraying Machine Setters, Operators, and Tenders \\ 
320 & 51-9121.02 & Coating, Painting, and Spraying Machine Operators and Tenders & 51-9121.00 & Coating, Painting, and Spraying Machine Setters, Operators, and Tenders \\ 
321 & 51-9131.00 & Photographic Process Workers & 51-9151.00 & Photographic Process Workers and Processing Machine Operators \\ 
322 & 51-9131.01 & Photographic Retouchers and Restorers & 51-9151.00 & Photographic Process Workers and Processing Machine Operators \\ 
323 & 51-9131.02 & Photographic Reproduction Technicians & 51-9151.00 & Photographic Process Workers and Processing Machine Operators \\ 
324 & 51-9131.03 & Photographic Hand Developers & 51-9151.00 & Photographic Process Workers and Processing Machine Operators \\ 
325 & 51-9131.04 & Film Laboratory Technicians & 51-9151.00 & Photographic Process Workers and Processing Machine Operators \\ 
326 & 51-9132.00 & Photographic Processing Machine Operators & 51-9151.00 & Photographic Process Workers and Processing Machine Operators \\ 
327 & 51-9194.01 & Precision Etchers and Engravers, Hand or Machine & 51-9194.00 & Etchers and Engravers \\ 
328 & 51-9194.02 & Engravers/Carvers & 51-9194.00 & Etchers and Engravers \\ 
329 & 51-9194.03 & Etchers & 51-9194.00 & Etchers and Engravers \\ 
330 & 51-9194.04 & Pantograph Engravers & 51-9194.00 & Etchers and Engravers \\ 
331 & 51-9194.05 & Etchers, Hand & 51-9194.00 & Etchers and Engravers \\ 
332 & 51-9194.06 & Engravers, Hand & 51-9194.00 & Etchers and Engravers \\ 
333 & 51-9195.01 & Precision Mold and Pattern Casters, Except Nonferrous Metals & 51-9195.07 & Molding and Casting Workers \\ 
334 & 51-9195.02 & Precision Pattern and Die Casters, Nonferrous Metals & 51-4072.00 & Molding, Coremaking, and Casting Machine Setters, Operators, and Tenders, Metal and Plastic \\ 
335 & 51-9195.06 & Mold Makers, Hand & 51-9195.07 & Molding and Casting Workers \\ 
336 & 51-9198.01 & Production Laborers & 51-9198.00 & Helpers--Production Workers \\ 
337 & 51-9198.02 & Production Helpers & 51-9198.00 & Helpers--Production Workers \\ 
338 & 51-9199.99 & Production Workers, All Other & 51-9199.00 &  \\ 
339 & 53-3032.01 & Truck Drivers, Heavy & 53-3032.00 & Heavy and Tractor-Trailer Truck Drivers \\ 
340 & 53-3032.02 & Tractor-Trailer Truck Drivers & 53-3032.00 & Heavy and Tractor-Trailer Truck Drivers \\ 
341 & 53-3099.99 & Motor Vehicle Operators, All Other & 53-3099.00 &  \\ 
342 & 53-4021.01 & Train Crew Members & 53-4021.00 & Railroad Brake, Signal, and Switch Operators \\ 
343 & 53-4021.02 & Railroad Yard Workers & 53-4021.00 & Railroad Brake, Signal, and Switch Operators \\ 
344 & 53-4099.99 & Rail Transportation Workers, All Other & 53-4099.00 &  \\ 
345 & 53-5011.01 & Able Seamen & 53-5011.00 & Sailors and Marine Oilers \\ 
346 & 53-5011.02 & Ordinary Seamen and Marine Oilers & 53-5011.00 & Sailors and Marine Oilers \\ 
347 & 53-6051.02 & Public Transportation Inspectors & 53-6051.07 & Transportation Vehicle, Equipment and Systems Inspectors, Except Aviation \\ 
348 & 53-6051.03 & Marine Cargo Inspectors & 53-6051.08 & Freight and Cargo Inspectors \\ 
349 & 53-6051.04 & Railroad Inspectors & 53-6051.07 & Transportation Vehicle, Equipment and Systems Inspectors, Except Aviation \\ 
350 & 53-6051.05 & Motor Vehicle Inspectors & 53-6051.07 & Transportation Vehicle, Equipment and Systems Inspectors, Except Aviation \\ 
351 & 53-6051.06 & Freight Inspectors & 53-6051.08 & Freight and Cargo Inspectors \\ 
352 & 53-6099.99 & Transportation Workers, All Other & 53-6099.00 &  \\ 
353 & 53-7032.01 & Excavating and Loading Machine Operators & 53-7032.00 & Excavating and Loading Machine and Dragline Operators \\ 
354 & 53-7032.02 & Dragline Operators & 53-7032.00 & Excavating and Loading Machine and Dragline Operators \\ 
355 & 53-7062.01 & Stevedores, Except Equipment Operators & 53-7062.00 & Laborers and Freight, Stock, and Material Movers, Hand \\ 
356 & 53-7062.02 & Grips and Set-Up Workers, Motion Picture Sets, Studios, and Stages & 53-7062.00 & Laborers and Freight, Stock, and Material Movers, Hand \\ 
357 & 53-7062.03 & Freight, Stock, and Material Movers, Hand & 53-7062.00 & Laborers and Freight, Stock, and Material Movers, Hand \\ 
358 & 53-7071.01 & Gas Pumping Station Operators & 53-7071.00 & Gas Compressor and Gas Pumping Station Operators \\ 
359 & 53-7071.02 & Gas Compressor Operators & 53-7071.00 & Gas Compressor and Gas Pumping Station Operators \\ 
360 & 53-7199.99 & Material Moving Workers, All Other & 53-7199.00 &  \\ 
361 & 55-1019.99 & Military Officer Special and Tactical Operations Leaders/Managers, All Other & 55-1019.00 &  \\ 
362 & 55-3019.99 & Military Enlisted Tactical Operations and Air/Weapons Specialists and Crew Members, All Other & 55-3019.00 &  \\ 
\hline \\[-1.8ex] 
\end{longtable} 

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
